Nonlinear Dimensionality Reduction with Diffusion Maps in Practice

Diffusion Map is a spectral dimensionality reduction technique which is able to uncover nonlinear submanifolds in high-dimensional data. And, it is increasingly applied across a wide range of scientific disciplines, such as biology, engineering, and social sciences. But data preprocessing, parameter settings and component selection have a significant influence on the resulting manifold, something which has not been comprehensively discussed in the literature so far. We provide a practice oriented review of the Diffusion Map technique, illustrate pitfalls and showcase a recently introduced technique for identifying the most relevant components. Our results show that the first components are not necessarily the most relevant ones.

==> intro.tex <==
%situation
In an increasingly connected and digitized  
world, the volume of complex, high-dimensional
data is growing rapidly across a broad range of disciplines, from biology, neuroscience, chemistry and physics, to social sciences. 
%
%problem
High dimensionality offers a deeper insight and potential of description, but it challenges the analysis, the visualization and the interpretation of the data.
%
%solution
Dimensionality reduction methods serve as essential tools for addressing these challenges, making such high-dimensional data more manageable by projecting it onto an interpretable low-dimensional space while preserving its essential structure. 


Standard approaches such as Principal Component Analysis (PCA) \cite{Pearson1901,Hotelling1933} and the Multidimensional Scaling method \cite{Torgerson1952,Ek2021} rely on linear transformations. They are very efficient, but are not able to capture nonlinear relationships prevalent in many real-world data sets. 
To capture such nonlinear patterns, non-linear dimensionality reduction methods need to be used. Here, spectral methods are particularly widespread. Examples are the Locally Linear Embedding \cite{roweis2000}, the Isomap \cite{Tenenbaum2000}, Spectral Clustering or Embedding \cite{Ng2001}, Kernel PCA \cite{schoelkopf1997}, Laplacian Eigenmaps \cite{Belkin2001} and the Diffusion Map \cite{lafon2004,Nadler2005,Coifman2006}. Notably, probabilistic perspectives on this type of technique had already been proposed earlier \cite{Meila2000,Meila2001}. However, earlier developments of this class of methods can also be found in the literature \cite{Scott1990,Weiss1999}. The core concept behind all these methods is rooted in the manifold hypothesis, which suggests that real-world datasets typically lie on a non-linear low-dimensional manifold embedded within the original high-dimensional space. Consequently, dimensionality reduction methods are also called manifold learning techniques. They aim to uncover this underlying structure, thereby enabling the construction of meaningful low-dimensional representations. Due to the conceptual similarities among these methods, several works have provided unified frameworks for nonlinear spectral techniques \cite{ham2004,Bengio2004,Strange2014,Ghojogh2023}.

The Diffusion Map method is a spectral dimensionality reduction method that offers a probabilistic interpretation based on the physics of diffusion \cite{Nadler2005}. 
And, it is increasingly applied across a wide range of scientific disciplines, including biology \cite{Xu2010,Fahimipour2020}, chemistry \cite{Ferguson2010, Kim2015,trstanova_2020}, engineering \cite{Bohn2013,Schwartz2014,Chen2016,Ghafourian2020}, geophysics \cite{Rabin2016,bregman_2021} and social sciences \cite{Le2013,Barter2019,Levin2021, Xiu2023,Xiu2024,Zeng2024,paula2024,Beier2025}.
%our problem 
But 
%However, a throughout and practice oriented review of the Diffusion Map technique is absent from the literature. In particular, we found the
data preprocessing, parameter settings and component selection have a significant influence on the resulting manifold, something which is seldomdiscussed in detail in the existing literature. Therefore, we provide a practice oriented review of the Diffusion Map technique, illustrating pitfalls and highlighting a recently introduced technique for selecting the most relevant components.

%here we come

%The paper pursues two main goals: (1) reviewing the Diffusion Map technique with detailed instructions for its use in practice and (2) introducing a quantitative method to assess the relevance of Diffusion Map components, based on neural networks.

The article is organized as follows. We first review the Diffusion Map method and  the associated computational algorithm. Next, we study its practical  properties -- the effect of different parameter settings and  the influence of data pre-processing -- with help of a standard example data set. We then discuss reasons when and why the most relevant component is not necessarily the first one, and end with reviewing a technique for quantifying the relevance of each component. %The conclusions are provided together with some perspectives in the final section.

%Specifically, we examine the effects of scaling individual variables, normalization procedures, and the presence of redundant variables, as well as the selection of the different Diffusion Map parameters. Furthermore, we explore methods for quantitatively assessing the relevance of Diffusion Map components. For that purpose, we propose an approach based on neural networks.\\
%nochmal schreiben wo was ist? Aber erst am Ende wenn alles fertig ist - Ja! :)

==> nre_scheme.tex <==
\begin{tikzpicture}[y=1cm, x=1cm, yscale=\globalscale,xscale=\globalscale, every node/.append style={scale=\globalscale}, inner sep=0pt, outer sep=0pt]
    \begin{scope}[shift={(-1.49, 0.98)}, >={latex[scale=3.0]}]
    \path[draw=black,line cap=round,line width=0.01cm] (3.0, 4.03) -- (3.0, 
  0.03) -- (6.0, 2.03) -- (6.0, 4.03) -- cycle;

    \path[draw=black,line cap=,line width=0.03cm] (6.8, 4.03) -- (6.8, 2.03);

    \path[draw=black,line cap=,line width=0.03cm] (2.2, 4.03) -- (2.2, 0.03);

    \path[draw=black,line cap=round,line width=0.01cm] (10.6, 4.03) -- (10.6, 
  0.03) -- (7.6, 2.03) -- (7.6, 4.03) -- cycle;

    \path[draw=black,line cap=,line width=0.03cm] (11.4, 4.04) -- (11.4, 0.04);

    \path[fill,line cap=round] (6.49, 3.12) -- (6.49, 3.04) -- (6.2, 
  3.04)arc(270.75:178.67:0.01 and -0.01)arc(180.74:89.26:0.01 and -0.01) -- 
  (6.49, 3.02) -- (6.49, 2.94) -- (6.65, 3.03) -- (6.49, 3.12) -- cycle;

    \node[text=black,align=center,anchor=south,line cap=round,line width=0.03cm, font=\small] (text11) at 
  (2.2, 4.33){original\\data};

    \node[text=black,align=center,anchor=south,line cap=round,line width=0.03cm, font=\small] (text13) at 
  (6.8, 4.46){embedding};

    \node[text=black,align=center,anchor=south,line cap=round,line width=0.03cm, font=\small] (text15) at 
  (11.41, 4.33){recon-\\struction};

    \node[text=black,align=center,anchor=center,line cap=round,line width=0.03cm, font=\normalsize] (text16) at 
  (4.5, 3.03){Diffusion\\Map};

    \node[text=black,align=center,anchor=center,line cap=round,line width=0.03cm, font=\normalsize] (text18) at 
  (9.1, 3.03){Neural\\Decoder};

    \node[text=black,anchor=base,line cap=round,line width=0.03cm] (text21) at 
  (2.21, -0.5){$x$};

    \node[text=black,anchor=south,line cap=round,line width=0.03cm] (text22) at 
  (6.8, 1.53){$\Psi(x)$};

    \node[text=black,anchor=base,line cap=round,line width=0.03cm] (text23) at 
  (11.4, -0.5){$\hat{\Psi}^{-1}(\Psi(x))$};

    \path[fill,line cap=round] (2.72, -0.2) -- (2.48, -0.34) -- (2.72, -0.48) --
   (2.72, -0.35) -- (10.06, -0.35) -- (10.06, -0.48) -- (10.30, -0.34) -- 
  (10.06, -0.2) -- (10.06, -0.32) -- (2.72, -0.32) -- (2.72, -0.2) -- cycle;

    \node[text=black,anchor=south,line cap=round,line width=0.03cm] (text29) at 
    (6.8, -0.84){\textbf{Neural Reconstruction Error}};

    \path[fill,line cap=round] (7.29, 3.12) -- (7.29, 3.04) -- (7.0, 
  3.04)arc(271.35:178.66:0.01 and -0.01)arc(180.75:88.67:0.01 and -0.01) -- 
  (7.29, 3.02) -- (7.29, 2.94) -- (7.45, 3.03) -- (7.29, 3.12) -- cycle;

    \path[fill,line cap=round] (11.09, 3.12) -- (11.09, 3.04) -- (10.8, 
  3.04)arc(270.75:178.67:0.01 and -0.01)arc(180.74:89.26:0.01 and -0.01) -- 
  (11.09, 3.02) -- (11.09, 2.94) -- (11.25, 3.03) -- (11.09, 3.12) -- cycle;

    \path[fill,line cap=round] (2.69, 3.12) -- (2.69, 3.04) -- (2.4, 
  3.04)arc(270.75:178.67:0.01 and -0.01)arc(180.74:89.26:0.01 and -0.01) -- 
  (2.69, 3.02) -- (2.69, 2.94) -- (2.85, 3.03) -- (2.69, 3.12) -- cycle;

  \end{scope}

\end{tikzpicture}


==> test <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{}
    \caption{}
    \label{}
\end{figure}
